Time-lagged Ordered Lasso for network inference

Accurate gene regulatory networks can be used to explain the emergence of different phenotypes, disease mechanisms, and other biological functions. Many methods have been proposed to infer networks from gene expression data but have been hampered by problems such as low sample size, inaccurate constraints, and incomplete characterizations of regulatory dynamics. Since expression regulation is dynamic, time-course data can be used to infer causality, but these datasets tend to be short or sparsely sampled. In addition, temporal methods typically assume that the expression of a gene at a time point depends on the expression of other genes at only the immediately preceding time point, while other methods include additional time points without any constraints to account for their temporal distance. These limitations can contribute to inaccurate networks with many missing and anomalous links. We adapted the time-lagged Ordered Lasso, a regularized regression method with temporal monotonicity constraints, for \textit{de novo} reconstruction. We also developed a semi-supervised method that embeds prior network information into the Ordered Lasso to discover novel regulatory dependencies in existing pathways. We evaluated these approaches on simulated data for a repressilator, time-course data from past DREAM challenges, and a HeLa cell cycle dataset to show that they can produce accurate networks subject to the dynamics and assumptions of the time-lagged Ordered Lasso regression.

==> acknowledgementsFunding.tex <==

%\section*{Acknowledgements}
\section*{Funding}

This work was supported by the James S.\, McDonnell Foundation (grant \#220020394) and the National Science Foundation (DMS-1547394).


==> title.tex <==
\subtitle{Gene expression} %or Systems biology?

\title[Time-lagged Ordered Lasso for network inference]{Time-lagged Ordered Lasso for network inference}
\author[Nguyen \textit{et~al}.]{Phan Nguyen\,$^{\text{\sfb 1}}$ and Rosemary Braun\,$^{\text{\sfb 1,2,*}}$}
\address{$^{\text{\sf 1}}$Department of Engineering Sciences and Applied Mathematics, Northwestern University, Evanston, IL 60208, USA\\
$^{\text{\sf 2}}$Biostatistics Division, Feinberg School of Medicine, Northwestern University, Chicago, IL 60611, USA}

\corresp{$^\ast$To whom correspondence should be addressed.}

\history{Received on XXXXX; revised on XXXXX; accepted on XXXXX}

\editor{Associate Editor: XXXXXXX}


